The Planck SZiFi catalogues: a new set of Planck catalogues of Sunyaev-Zeldovich-detected galaxy clusters

We introduce the Planck SZiFi catalogues, a new set of 10 catalogues of galaxy clusters detected through their thermal Sunyaev-Zeldovich (tSZ) signature. The catalogues are produced by applying the SZiFi cluster finder to the Planck PR3 temperature data down to a signal-to-noise threshold of 5. They span three frequency channel combinations (100-857 GHz, 100-545 GHz, and 100-353 GHz) and 7 of them are constructed by spectrally deprojecting the Cosmic Infrared Background (CIB). This approach allows us, for the first time in the context of cluster finding, to carefully assess the impact of the cluster-correlated CIB on the recovered cluster tSZ observables, which we find to be negligible. In addition, we quantify the impact of the relativistic corrections to the tSZ signal, finding them to be at the 5-10% level for the cluster tSZ amplitude but negligible for the signal-to-noise. We compile our catalogues into a single Planck SZiFi master catalogue containing a total of 1499 detections. We cross-match the master catalogue with several external tSZ and X-ray cluster catalogues, setting a lower bound on the purity of our baseline catalogue of 95% and 99% at a minimum signal-to-noise of 5 and 6, respectively. We validate our cluster detection pipeline by applying it to synthetic observations, recovering cluster number counts for which we are able to produce a theoretical prediction that accurately describes them. This validation exercise indicates that our catalogues are well-suited for cosmological inference. The Planck SZiFi master catalogue will become publicly available at github.com/inigozubeldia/szifi/tree/main/planck_szifi_master_catalogue.

==> Planck_catalogue_paper-2 <==
\begin{thebibliography}{}
\makeatletter
\relax
\def\mn@urlcharsother{\let\do\@makeother \do\$\do\&\do\#\do\^\do\_\do\%\do\~}
\def\mn@doi{\begingroup\mn@urlcharsother \@ifnextchar [ {\mn@doi@} {\mn@doi@[]}}
\def\mn@doi@[#1]#2{\def\@tempa{#1}\ifx\@tempa\@empty \href {http://dx.doi.org/#2} {doi:#2}\else \href {http://dx.doi.org/#2} {#1}\fi \endgroup}
\def\mn@eprint#1#2{\mn@eprint@#1:#2::\@nil}
\def\mn@eprint@arXiv#1{\href {http://arxiv.org/abs/#1} {{\tt arXiv:#1}}}
\def\mn@eprint@dblp#1{\href {http://dblp.uni-trier.de/rec/bibtex/#1.xml} {dblp:#1}}
\def\mn@eprint@#1:#2:#3:#4\@nil{\def\@tempa {#1}\def\@tempb {#2}\def\@tempc {#3}\ifx \@tempc \@empty \let \@tempc \@tempb \let \@tempb \@tempa \fi \ifx \@tempb \@empty \def\@tempb {arXiv}\fi \@ifundefined {mn@eprint@\@tempb}{\@tempb:\@tempc}{\expandafter \expandafter \csname mn@eprint@\@tempb\endcsname \expandafter{\@tempc}}}

\bibitem[\protect\citeauthoryear{{Aghanim} et~al.,}{{Aghanim} et~al.}{2019}]{Aghanim2019}
{Aghanim} N.,  et~al., 2019, \mn@doi [\aap] {10.1051/0004-6361/201935271}, \href {https://ui.adsabs.harvard.edu/abs/2019A&A...632A..47A} {632, A47}

\bibitem[\protect\citeauthoryear{{Aguado-Barahona}, {Barrena}, {Streblyanska}, {Ferragamo}, {Rubi{\~n}o-Mart{\'\i}n}, {Tramonte}  \& {Lietzen}}{{Aguado-Barahona} et~al.}{2019}]{Aguado-Barahona2019}
{Aguado-Barahona} A.,  {Barrena} R.,  {Streblyanska} A.,  {Ferragamo} A.,  {Rubi{\~n}o-Mart{\'\i}n} J.~A.,  {Tramonte} D.,   {Lietzen} H.,  2019, \mn@doi [\aap] {10.1051/0004-6361/201936034}, \href {https://ui.adsabs.harvard.edu/abs/2019A&A...631A.148A} {631, A148}

\bibitem[\protect\citeauthoryear{{Allen}, {Evrard}  \& {Mantz}}{{Allen} et~al.}{2011}]{Allen2011}
{Allen} S.~W.,  {Evrard} A.~E.,   {Mantz} A.~B.,  2011, \mn@doi [\araa] {10.1146/annurev-astro-081710-102514}, \href {http://adsabs.harvard.edu/abs/2011ARA%26A..49..409A} {49, 409}

\bibitem[\protect\citeauthoryear{{Alonso}, {Sanchez}, {Slosar}  \& {LSST Dark Energy Science Collaboration}}{{Alonso} et~al.}{2019}]{Alonso2019}
{Alonso} D.,  {Sanchez} J.,  {Slosar} A.,   {LSST Dark Energy Science Collaboration} 2019, \mn@doi [\mnras] {10.1093/mnras/stz093}, \href {https://ui.adsabs.harvard.edu/abs/2019MNRAS.484.4127A} {484, 4127}

\bibitem[\protect\citeauthoryear{{Amodeo} et~al.,}{{Amodeo} et~al.}{2018}]{Amodeo2018}
{Amodeo} S.,  et~al., 2018, \mn@doi [\apj] {10.3847/1538-4357/aa98dd}, \href {https://ui.adsabs.harvard.edu/abs/2018ApJ...853...36A} {853, 36}

\bibitem[\protect\citeauthoryear{{Arnaud}, {Pratt}, {Piffaretti}, {B{\"o}hringer}, {Croston}  \& {Pointecouteau}}{{Arnaud} et~al.}{2010}]{Arnaud2010}
{Arnaud} M.,  {Pratt} G.~W.,  {Piffaretti} R.,  {B{\"o}hringer} H.,  {Croston} J.~H.,   {Pointecouteau} E.,  2010, \mn@doi [\aap] {10.1051/0004-6361/200913416}, \href {http://adsabs.harvard.edu/abs/2010A%26A...517A..92A} {517, A92}

\bibitem[\protect\citeauthoryear{{Barrena} et~al.,}{{Barrena} et~al.}{2018}]{Barrena2018}
{Barrena} R.,  et~al., 2018, \mn@doi [\aap] {10.1051/0004-6361/201732315}, \href {https://ui.adsabs.harvard.edu/abs/2018A&A...616A..42B} {616, A42}

\bibitem[\protect\citeauthoryear{{Barrena} et~al.,}{{Barrena} et~al.}{2020}]{Barrena2020}
{Barrena} R.,  et~al., 2020, \mn@doi [\aap] {10.1051/0004-6361/202037552}, \href {https://ui.adsabs.harvard.edu/abs/2020A&A...638A.146B} {638, A146}

\bibitem[\protect\citeauthoryear{Battye \& Weller}{Battye \& Weller}{2003}]{Battye:2003bm}
Battye R.~A.,  Weller J.,  2003, \mn@doi [Phys. Rev. D] {10.1103/PhysRevD.68.083506}, 68, 083506

\bibitem[\protect\citeauthoryear{{Bleem}, {Stalder}, {de Haan}  et~al.}{{Bleem} et~al.}{2015}]{Bleem2015}
{Bleem} L.~E.,  {Stalder} B.,  {de Haan} T.,   et~al., 2015, \mn@doi [\apjs] {10.1088/0067-0049/216/2/27}, \href {http://adsabs.harvard.edu/abs/2015ApJS..216...27B} {216, 27}

\bibitem[\protect\citeauthoryear{{Bleem} et~al.,}{{Bleem} et~al.}{2020}]{Bleem2020}
{Bleem} L.~E.,  et~al., 2020, \mn@doi [\apjs] {10.3847/1538-4365/ab6993}, \href {https://ui.adsabs.harvard.edu/abs/2020ApJS..247...25B} {247, 25}

\bibitem[\protect\citeauthoryear{{Bleem} et~al.,}{{Bleem} et~al.}{2022}]{Bleem2022}
{Bleem} L.~E.,  et~al., 2022, \mn@doi [\apjs] {10.3847/1538-4365/ac35e9}, \href {https://ui.adsabs.harvard.edu/abs/2022ApJS..258...36B} {258, 36}

\bibitem[\protect\citeauthoryear{{Bleem} et~al.,}{{Bleem} et~al.}{2024}]{Bleem2024}
{Bleem} L.~E.,  et~al., 2024, \mn@doi [The Open Journal of Astrophysics] {10.21105/astro.2311.07512}, \href {https://ui.adsabs.harvard.edu/abs/2024OJAp....7E..13B} {7, 13}

\bibitem[\protect\citeauthoryear{{Boada}, {Hughes}, {Menanteau}, {Doze}, {Barrientos}  \& {Infante}}{{Boada} et~al.}{2019}]{Boada2019}
{Boada} S.,  {Hughes} J.~P.,  {Menanteau} F.,  {Doze} P.,  {Barrientos} L.~F.,   {Infante} L.,  2019, \mn@doi [\apj] {10.3847/1538-4357/aaf3a0}, \href {https://ui.adsabs.harvard.edu/abs/2019ApJ...871..188B} {871, 188}

\bibitem[\protect\citeauthoryear{{Bocquet}, {Dietrich}, {Schrabback}, {Bleem}, {Klein}  et~al.}{{Bocquet} et~al.}{2019}]{Bocquet2018}
{Bocquet} S.,  {Dietrich} J.~P.,  {Schrabback} T.,  {Bleem} L.~E.,  {Klein} M.,   et~al., 2019, \mn@doi [\apj] {10.3847/1538-4357/ab1f10}, \href {https://ui.adsabs.harvard.edu/abs/2019ApJ...878...55B} {878, 55}

\bibitem[\protect\citeauthoryear{{Bocquet} et~al.,}{{Bocquet} et~al.}{2023}]{Bocquet2023}
{Bocquet} S.,  et~al., 2023, \mn@doi [arXiv e-prints] {10.48550/arXiv.2310.12213}, \href {https://ui.adsabs.harvard.edu/abs/2023arXiv231012213B} {p. arXiv:2310.12213}

\bibitem[\protect\citeauthoryear{{Bocquet} et~al.,}{{Bocquet} et~al.}{2024}]{Bocquet2024}
{Bocquet} S.,  et~al., 2024, \mn@doi [arXiv e-prints] {10.48550/arXiv.2401.02075}, \href {https://ui.adsabs.harvard.edu/abs/2024arXiv240102075B} {p. arXiv:2401.02075}

\bibitem[\protect\citeauthoryear{{B{\"o}hringer} et~al.,}{{B{\"o}hringer} et~al.}{2000}]{Bohringer2000}
{B{\"o}hringer} H.,  et~al., 2000, \mn@doi [\apjs] {10.1086/313427}, \href {https://ui.adsabs.harvard.edu/abs/2000ApJS..129..435B} {129, 435}

\bibitem[\protect\citeauthoryear{{Bolliet}, {Spurio Mancini}, {Hill}, {Madhavacheril}, {Jense}, {Calabrese}  \& {Dunkley}}{{Bolliet} et~al.}{2023}]{Bolliet2023}
{Bolliet} B.,  {Spurio Mancini} A.,  {Hill} J.~C.,  {Madhavacheril} M.,  {Jense} H.~T.,  {Calabrese} E.,   {Dunkley} J.,  2023, \mn@doi [arXiv e-prints] {10.48550/arXiv.2303.01591}, \href {https://ui.adsabs.harvard.edu/abs/2023arXiv230301591B} {p. arXiv:2303.01591}

\bibitem[\protect\citeauthoryear{{Bulbul} et~al.,}{{Bulbul} et~al.}{2024}]{Bulbul2024}
{Bulbul} E.,  et~al., 2024, \mn@doi [\aap] {10.1051/0004-6361/202348264}, \href {https://ui.adsabs.harvard.edu/abs/2024A&A...685A.106B} {685, A106}

\bibitem[\protect\citeauthoryear{{Burenin}, {Vikhlinin}, {Hornstrup}, {Ebeling}, {Quintana}  \& {Mescheryakov}}{{Burenin} et~al.}{2007}]{Burenin2007}
{Burenin} R.~A.,  {Vikhlinin} A.,  {Hornstrup} A.,  {Ebeling} H.,  {Quintana} H.,   {Mescheryakov} A.,  2007, \mn@doi [\apjs] {10.1086/519457}, \href {https://ui.adsabs.harvard.edu/abs/2007ApJS..172..561B} {172, 561}

\bibitem[\protect\citeauthoryear{{Burenin} et~al.,}{{Burenin} et~al.}{2018}]{Burenin2018}
{Burenin} R.~A.,  et~al., 2018, \mn@doi [Astronomy Letters] {10.1134/S1063773718050018}, \href {https://ui.adsabs.harvard.edu/abs/2018AstL...44..297B} {44, 297}

\bibitem[\protect\citeauthoryear{{Burke}, {Collins}, {Sharples}, {Romer}  \& {Nichol}}{{Burke} et~al.}{2003}]{Burke2003}
{Burke} D.~J.,  {Collins} C.~A.,  {Sharples} R.~M.,  {Romer} A.~K.,   {Nichol} R.~C.,  2003, \mn@doi [\mnras] {10.1046/j.1365-8711.2003.06378.x}, \href {https://ui.adsabs.harvard.edu/abs/2003MNRAS.341.1093B} {341, 1093}

\bibitem[\protect\citeauthoryear{Carlstrom, Holder  \& Reese}{Carlstrom et~al.}{2002}]{Carlstrom2002}
Carlstrom J.~E.,  Holder G.~P.,   Reese E.~D.,  2002, \mn@doi [Annual Review of Astronomy and Astrophysics] {10.1146/annurev.astro.40.060401.093803}, 40, 643–680

\bibitem[\protect\citeauthoryear{{Challinor} \& {Lasenby}}{{Challinor} \& {Lasenby}}{1998}]{Challinor1998}
{Challinor} A.,  {Lasenby} A.,  1998, \mn@doi [\apj] {10.1086/305623}, \href {https://ui.adsabs.harvard.edu/abs/1998ApJ...499....1C} {499, 1}

\bibitem[\protect\citeauthoryear{{Chaubal} et~al.,}{{Chaubal} et~al.}{2022}]{Chaubal2022}
{Chaubal} P.~S.,  et~al., 2022, \mn@doi [\apj] {10.3847/1538-4357/ac6a55}, \href {https://ui.adsabs.harvard.edu/abs/2022ApJ...931..139C} {931, 139}

\bibitem[\protect\citeauthoryear{{Chluba}, {Nagai}, {Sazonov}  \& {Nelson}}{{Chluba} et~al.}{2012}]{Chluba2012SZpack}
{Chluba} J.,  {Nagai} D.,  {Sazonov} S.,   {Nelson} K.,  2012, \mn@doi [\mnras] {10.1111/j.1365-2966.2012.21741.x}, \href {http://adsabs.harvard.edu/abs/2012MNRAS.426..510C} {426, 510}

\bibitem[\protect\citeauthoryear{{Chluba}, {Switzer}, {Nelson}  \& {Nagai}}{{Chluba} et~al.}{2013}]{Chluba2013}
{Chluba} J.,  {Switzer} E.,  {Nelson} K.,   {Nagai} D.,  2013, \mn@doi [\mnras] {10.1093/mnras/stt110}, \href {https://ui.adsabs.harvard.edu/abs/2013MNRAS.430.3054C} {430, 3054}

\bibitem[\protect\citeauthoryear{{Chluba}, {Hill}  \& {Abitbol}}{{Chluba} et~al.}{2017}]{Chluba2017}
{Chluba} J.,  {Hill} J.~C.,   {Abitbol} M.~H.,  2017, \mn@doi [\mnras] {10.1093/mnras/stx1982}, \href {https://ui.adsabs.harvard.edu/abs/2017MNRAS.472.1195C} {472, 1195}

\bibitem[\protect\citeauthoryear{{Chon} \& {B{\"o}hringer}}{{Chon} \& {B{\"o}hringer}}{2012}]{Chon2012}
{Chon} G.,  {B{\"o}hringer} H.,  2012, \mn@doi [\aap] {10.1051/0004-6361/201117996}, \href {https://ui.adsabs.harvard.edu/abs/2012A&A...538A..35C} {538, A35}

\bibitem[\protect\citeauthoryear{{Coulton} et~al.,}{{Coulton} et~al.}{2024}]{Coulton2024}
{Coulton} W.,  et~al., 2024, \mn@doi [\prd] {10.1103/PhysRevD.109.063530}, \href {https://ui.adsabs.harvard.edu/abs/2024PhRvD.109f3530C} {109, 063530}

\bibitem[\protect\citeauthoryear{{Cruddace} et~al.,}{{Cruddace} et~al.}{2002}]{Cruddace2002}
{Cruddace} R.,  et~al., 2002, \mn@doi [\apjs] {10.1086/324519}, \href {https://ui.adsabs.harvard.edu/abs/2002ApJS..140..239C} {140, 239}

\bibitem[\protect\citeauthoryear{{Delabrouille}, {Cardoso}, {Le Jeune}, {Betoule}, {Fay}  \& {Guilloux}}{{Delabrouille} et~al.}{2009}]{Delabrouille2009}
{Delabrouille} J.,  {Cardoso} J.~F.,  {Le Jeune} M.,  {Betoule} M.,  {Fay} G.,   {Guilloux} F.,  2009, \mn@doi [\aap] {10.1051/0004-6361:200810514}, \href {https://ui.adsabs.harvard.edu/abs/2009A&A...493..835D} {493, 835}

\bibitem[\protect\citeauthoryear{{Ebeling}, {Edge}, {Bohringer}, {Allen}, {Crawford}, {Fabian}, {Voges}  \& {Huchra}}{{Ebeling} et~al.}{1998}]{Ebeling1998}
{Ebeling} H.,  {Edge} A.~C.,  {Bohringer} H.,  {Allen} S.~W.,  {Crawford} C.~S.,  {Fabian} A.~C.,  {Voges} W.,   {Huchra} J.~P.,  1998, \mn@doi [\mnras] {10.1046/j.1365-8711.1998.01949.x}, \href {https://ui.adsabs.harvard.edu/abs/1998MNRAS.301..881E} {301, 881}

\bibitem[\protect\citeauthoryear{{Ebeling}, {Edge}, {Allen}, {Crawford}, {Fabian}  \& {Huchra}}{{Ebeling} et~al.}{2000}]{Ebeling2000}
{Ebeling} H.,  {Edge} A.~C.,  {Allen} S.~W.,  {Crawford} C.~S.,  {Fabian} A.~C.,   {Huchra} J.~P.,  2000, \mn@doi [\mnras] {10.1046/j.1365-8711.2000.03549.x}, \href {https://ui.adsabs.harvard.edu/abs/2000MNRAS.318..333E} {318, 333}

\bibitem[\protect\citeauthoryear{{Ebeling}, {Mullis}  \& {Tully}}{{Ebeling} et~al.}{2002}]{Ebeling2002}
{Ebeling} H.,  {Mullis} C.~R.,   {Tully} R.~B.,  2002, \mn@doi [\apj] {10.1086/343790}, \href {https://ui.adsabs.harvard.edu/abs/2002ApJ...580..774E} {580, 774}

\bibitem[\protect\citeauthoryear{{Ebeling}, {Barrett}, {Donovan}, {Ma}, {Edge}  \& {van Speybroeck}}{{Ebeling} et~al.}{2007}]{Ebeling2007}
{Ebeling} H.,  {Barrett} E.,  {Donovan} D.,  {Ma} C.~J.,  {Edge} A.~C.,   {van Speybroeck} L.,  2007, \mn@doi [\apjl] {10.1086/518603}, \href {https://ui.adsabs.harvard.edu/abs/2007ApJ...661L..33E} {661, L33}

\bibitem[\protect\citeauthoryear{{Erler}, {Basu}, {Chluba}  \& {Bertoldi}}{{Erler} et~al.}{2018}]{Erler2018}
{Erler} J.,  {Basu} K.,  {Chluba} J.,   {Bertoldi} F.,  2018, \mn@doi [\mnras] {10.1093/mnras/sty327}, \href {https://ui.adsabs.harvard.edu/abs/2018MNRAS.476.3360E} {476, 3360}

\bibitem[\protect\citeauthoryear{{Finoguenov} et~al.,}{{Finoguenov} et~al.}{2020}]{Finoguenov2020}
{Finoguenov} A.,  et~al., 2020, \mn@doi [\aap] {10.1051/0004-6361/201937283}, \href {https://ui.adsabs.harvard.edu/abs/2020A&A...638A.114F} {638, A114}

\bibitem[\protect\citeauthoryear{{Giard}, {Montier}, {Pointecouteau}  \& {Simmat}}{{Giard} et~al.}{2008}]{Giard2008}
{Giard} M.,  {Montier} L.,  {Pointecouteau} E.,   {Simmat} E.,  2008, \mn@doi [\aap] {10.1051/0004-6361:200810442}, \href {https://ui.adsabs.harvard.edu/abs/2008A&A...490..547G} {490, 547}

\bibitem[\protect\citeauthoryear{{Gioia} \& {Luppino}}{{Gioia} \& {Luppino}}{1994}]{Gioia1994}
{Gioia} I.~M.,  {Luppino} G.~A.,  1994, \mn@doi [\apjs] {10.1086/192083}, \href {https://ui.adsabs.harvard.edu/abs/1994ApJS...94..583G} {94, 583}

\bibitem[\protect\citeauthoryear{{G{\'o}rski}, {Hivon}, {Banday}, {Wandelt}, {Hansen}, {Reinecke}  \& {Bartelmann}}{{G{\'o}rski} et~al.}{2005}]{Gorski2005}
{G{\'o}rski} K.~M.,  {Hivon} E.,  {Banday} A.~J.,  {Wandelt} B.~D.,  {Hansen} F.~K.,  {Reinecke} M.,   {Bartelmann} M.,  2005, \mn@doi [\apj] {10.1086/427976}, \href {http://adsabs.harvard.edu/abs/2005ApJ...622..759G} {622, 759}

\bibitem[\protect\citeauthoryear{{Gruetjen}, {Fergusson}, {Liguori}  \& {Shellard}}{{Gruetjen} et~al.}{2017}]{Gruetjen2015}
{Gruetjen} H.~F.,  {Fergusson} J.~R.,  {Liguori} M.,   {Shellard} E.~P.~S.,  2017, \mn@doi [\prd] {10.1103/PhysRevD.95.043532}, \href {http://adsabs.harvard.edu/abs/2017PhRvD..95d3532G} {95, 043532}

\bibitem[\protect\citeauthoryear{{Hasselfield}, {Hilton}, {Marriage}  et~al.}{{Hasselfield} et~al.}{2013}]{Hasselfield2013}
{Hasselfield} M.,  {Hilton} M.,  {Marriage} T.~A.,   et~al., 2013, \mn@doi [\jcap] {10.1088/1475-7516/2013/07/008}, \href {http://adsabs.harvard.edu/abs/2013JCAP...07..008H} {7, 008}

\bibitem[\protect\citeauthoryear{{Henry}}{{Henry}}{2004}]{Henry2004bb}
{Henry} J.~P.,  2004, \mn@doi [\apj] {10.1086/421336}, \href {https://ui.adsabs.harvard.edu/abs/2004ApJ...609..603H} {609, 603}

\bibitem[\protect\citeauthoryear{{Henry}, {Mullis}, {Voges}, {B{\"o}hringer}, {Briel}, {Gioia}  \& {Huchra}}{{Henry} et~al.}{2006}]{Henry2006}
{Henry} J.~P.,  {Mullis} C.~R.,  {Voges} W.,  {B{\"o}hringer} H.,  {Briel} U.~G.,  {Gioia} I.~M.,   {Huchra} J.~P.,  2006, \mn@doi [\apjs] {10.1086/498749}, \href {https://ui.adsabs.harvard.edu/abs/2006ApJS..162..304H} {162, 304}

\bibitem[\protect\citeauthoryear{{Herranz}, {Sanz}, {Hobson}, {Barreiro}, {Diego}, {Mart{\'\i}nez-Gonz{\'a}lez}  \& {Lasenby}}{{Herranz} et~al.}{2002}]{Herranz2002}
{Herranz} D.,  {Sanz} J.~L.,  {Hobson} M.~P.,  {Barreiro} R.~B.,  {Diego} J.~M.,  {Mart{\'\i}nez-Gonz{\'a}lez} E.,   {Lasenby} A.~N.,  2002, \mn@doi [\mnras] {10.1046/j.1365-8711.2002.05704.x}, \href {https://ui.adsabs.harvard.edu/abs/2002MNRAS.336.1057H} {336, 1057}

\bibitem[\protect\citeauthoryear{{Hilton}, {Hasselfield}, {Sif{\'o}n}, {Battaglia}  et~al.}{{Hilton} et~al.}{2018}]{Hilton2018}
{Hilton} M.,  {Hasselfield} M.,  {Sif{\'o}n} C.,  {Battaglia} N.,   et~al., 2018, \mn@doi [\apjs] {10.3847/1538-4365/aaa6cb}, \href {https://ui.adsabs.harvard.edu/abs/2018ApJS..235...20H} {235, 20}

\bibitem[\protect\citeauthoryear{{Hilton} et~al.,}{{Hilton} et~al.}{2021}]{Hilton2020}
{Hilton} M.,  et~al., 2021, \mn@doi [\apjs] {10.3847/1538-4365/abd023}, \href {https://ui.adsabs.harvard.edu/abs/2021ApJS..253....3H} {253, 3}

\bibitem[\protect\citeauthoryear{{Hivon}, {G{\'o}rski}, {Netterfield}, {Crill}, {Prunet}  \& {Hansen}}{{Hivon} et~al.}{2002}]{Hivon2002}
{Hivon} E.,  {G{\'o}rski} K.~M.,  {Netterfield} C.~B.,  {Crill} B.~P.,  {Prunet} S.,   {Hansen} F.,  2002, \mn@doi [\apj] {10.1086/338126}, \href {https://ui.adsabs.harvard.edu/abs/2002ApJ...567....2H} {567, 2}

\bibitem[\protect\citeauthoryear{{Horner}, {Perlman}, {Ebeling}, {Jones}, {Scharf}, {Wegner}, {Malkan}  \& {Maughan}}{{Horner} et~al.}{2008}]{Horner2008}
{Horner} D.~J.,  {Perlman} E.~S.,  {Ebeling} H.,  {Jones} L.~R.,  {Scharf} C.~A.,  {Wegner} G.,  {Malkan} M.,   {Maughan} B.,  2008, \mn@doi [\apjs] {10.1086/529494}, \href {https://ui.adsabs.harvard.edu/abs/2008ApJS..176..374H} {176, 374}

\bibitem[\protect\citeauthoryear{{Hurier} \& {Lacasa}}{{Hurier} \& {Lacasa}}{2017}]{Hurier2017}
{Hurier} G.,  {Lacasa} F.,  2017, \mn@doi [\aap] {10.1051/0004-6361/201630041}, \href {https://ui.adsabs.harvard.edu/abs/2017A%26A...604A..71H} {604, A71}

\bibitem[\protect\citeauthoryear{{Itoh}, {Kohyama}  \& {Nozawa}}{{Itoh} et~al.}{1998}]{Itoh1998}
{Itoh} N.,  {Kohyama} Y.,   {Nozawa} S.,  1998, \mn@doi [\apj] {10.1086/305876}, \href {https://ui.adsabs.harvard.edu/abs/1998ApJ...502....7I} {502, 7}

\bibitem[\protect\citeauthoryear{{Klein}, {Hern{\'a}ndez-Lang}, {Mohr}, {Bocquet}  \& {Singh}}{{Klein} et~al.}{2023}]{Klein2023}
{Klein} M.,  {Hern{\'a}ndez-Lang} D.,  {Mohr} J.~J.,  {Bocquet} S.,   {Singh} A.,  2023, \mn@doi [\mnras] {10.1093/mnras/stad2729}, \href {https://ui.adsabs.harvard.edu/abs/2023MNRAS.526.3757K} {526, 3757}

\bibitem[\protect\citeauthoryear{{Kocevski}, {Ebeling}, {Mullis}  \& {Tully}}{{Kocevski} et~al.}{2007}]{Kocevski2007}
{Kocevski} D.~D.,  {Ebeling} H.,  {Mullis} C.~R.,   {Tully} R.~B.,  2007, \mn@doi [\apj] {10.1086/513303}, \href {https://ui.adsabs.harvard.edu/abs/2007ApJ...662..224K} {662, 224}

\bibitem[\protect\citeauthoryear{{Lagache}, {Puget}  \& {Dole}}{{Lagache} et~al.}{2005}]{Lagache2005}
{Lagache} G.,  {Puget} J.-L.,   {Dole} H.,  2005, \mn@doi [\araa] {10.1146/annurev.astro.43.072103.150606}, \href {https://ui.adsabs.harvard.edu/abs/2005ARA&A..43..727L} {43, 727}

\bibitem[\protect\citeauthoryear{{Lee}, {Chluba}, {Kay}  \& {Barnes}}{{Lee} et~al.}{2020}]{Lee2020}
{Lee} E.,  {Chluba} J.,  {Kay} S.~T.,   {Barnes} D.~J.,  2020, \mn@doi [\mnras] {10.1093/mnras/staa450}, \href {https://ui.adsabs.harvard.edu/abs/2020MNRAS.493.3274L} {493, 3274}

\bibitem[\protect\citeauthoryear{{Lee} et~al.,}{{Lee} et~al.}{2022}]{Lee2022}
{Lee} E.,  et~al., 2022, \mn@doi [\mnras] {10.1093/mnras/stac2781}, \href {https://ui.adsabs.harvard.edu/abs/2022MNRAS.517.5303L} {517, 5303}

\bibitem[\protect\citeauthoryear{{Lee}, {Battye}  \& {Bolliet}}{{Lee} et~al.}{2024}]{Lee2024}
{Lee} E.,  {Battye} R.,   {Bolliet} B.,  2024, \mn@doi [arXiv e-prints] {10.48550/arXiv.2403.19542}, \href {https://ui.adsabs.harvard.edu/abs/2024arXiv240319542L} {p. arXiv:2403.19542}

\bibitem[\protect\citeauthoryear{{Mann} \& {Ebeling}}{{Mann} \& {Ebeling}}{2012}]{Mann2012}
{Mann} A.~W.,  {Ebeling} H.,  2012, \mn@doi [\mnras] {10.1111/j.1365-2966.2011.20170.x}, \href {https://ui.adsabs.harvard.edu/abs/2012MNRAS.420.2120M} {420, 2120}

\bibitem[\protect\citeauthoryear{{Mantz}, {Allen}, {Ebeling}, {Rapetti}  \& {Drlica-Wagner}}{{Mantz} et~al.}{2010}]{Mantz2010b}
{Mantz} A.,  {Allen} S.~W.,  {Ebeling} H.,  {Rapetti} D.,   {Drlica-Wagner} A.,  2010, \mn@doi [\mnras] {10.1111/j.1365-2966.2010.16993.x}, \href {https://ui.adsabs.harvard.edu/abs/2010MNRAS.406.1773M} {406, 1773}

\bibitem[\protect\citeauthoryear{{Marriage} et~al.,}{{Marriage} et~al.}{2011}]{Marriage2011}
{Marriage} T.~A.,  et~al., 2011, \mn@doi [\apj] {10.1088/0004-637X/737/2/61}, \href {https://ui.adsabs.harvard.edu/abs/2011ApJ...737...61M} {737, 61}

\bibitem[\protect\citeauthoryear{{McCarthy} \& {Hill}}{{McCarthy} \& {Hill}}{2024a}]{McCarthy2024}
{McCarthy} F.,  {Hill} J.~C.,  2024a, \mn@doi [\prd] {10.1103/PhysRevD.109.023528}, \href {https://ui.adsabs.harvard.edu/abs/2024PhRvD.109b3528M} {109, 023528}

\bibitem[\protect\citeauthoryear{{McCarthy} \& {Hill}}{{McCarthy} \& {Hill}}{2024b}]{McCarthy2024b}
{McCarthy} F.,  {Hill} J.~C.,  2024b, \mn@doi [\prd] {10.1103/PhysRevD.109.023529}, \href {https://ui.adsabs.harvard.edu/abs/2024PhRvD.109b3529M} {109, 023529}

\bibitem[\protect\citeauthoryear{{Melin}, {Bartlett}  \& {Delabrouille}}{{Melin} et~al.}{2006}]{Melin2006}
{Melin} J.~B.,  {Bartlett} J.~G.,   {Delabrouille} J.,  2006, \mn@doi [\aap] {10.1051/0004-6361:20065034}, \href {https://ui.adsabs.harvard.edu/abs/2006A&A...459..341M} {459, 341}

\bibitem[\protect\citeauthoryear{{Melin}, {Bartlett}, {Cai}, {De Zotti}, {Delabrouille}, {Roman}  \& {Bonaldi}}{{Melin} et~al.}{2018}]{Melin2018}
{Melin} J.~B.,  {Bartlett} J.~G.,  {Cai} Z.~Y.,  {De Zotti} G.,  {Delabrouille} J.,  {Roman} M.,   {Bonaldi} A.,  2018, \mn@doi [\aap] {10.1051/0004-6361/201732292}, \href {https://ui.adsabs.harvard.edu/abs/2018A&A...617A..75M} {617, A75}

\bibitem[\protect\citeauthoryear{{Melin}, {Bartlett}, {Tarr{\'\i}o}  \& {Pratt}}{{Melin} et~al.}{2021}]{Melin2021}
{Melin} J.~B.,  {Bartlett} J.~G.,  {Tarr{\'\i}o} P.,   {Pratt} G.~W.,  2021, \mn@doi [\aap] {10.1051/0004-6361/202039471}, \href {https://ui.adsabs.harvard.edu/abs/2021A&A...647A.106M} {647, A106}

\bibitem[\protect\citeauthoryear{{Montier} \& {Giard}}{{Montier} \& {Giard}}{2005}]{Montier2005}
{Montier} L.~A.,  {Giard} M.,  2005, \mn@doi [\aap] {10.1051/0004-6361:20042388}, \href {https://ui.adsabs.harvard.edu/abs/2005A&A...439...35M} {439, 35}

\bibitem[\protect\citeauthoryear{{Mroczkowski}, {Nagai}  et~al.}{{Mroczkowski} et~al.}{2019}]{Mroczkowski2019}
{Mroczkowski} T.,  {Nagai} D.,   et~al., 2019, \mn@doi [\ssr] {10.1007/s11214-019-0581-2}, \href {https://ui.adsabs.harvard.edu/abs/2019SSRv..215...17M} {215, 17}

\bibitem[\protect\citeauthoryear{{Mullis} et~al.,}{{Mullis} et~al.}{2003}]{Mullis2003}
{Mullis} C.~R.,  et~al., 2003, \mn@doi [\apj] {10.1086/376866}, \href {https://ui.adsabs.harvard.edu/abs/2003ApJ...594..154M} {594, 154}

\bibitem[\protect\citeauthoryear{{Nagai}, {Kravtsov}  \& {Vikhlinin}}{{Nagai} et~al.}{2007}]{Nagai2007}
{Nagai} D.,  {Kravtsov} A.~V.,   {Vikhlinin} A.,  2007, \mn@doi [\apj] {10.1086/521328}, \href {http://adsabs.harvard.edu/abs/2007ApJ...668....1N} {668, 1}

\bibitem[\protect\citeauthoryear{{Pandey} et~al.,}{{Pandey} et~al.}{2019}]{Pandey2019}
{Pandey} S.,  et~al., 2019, \mn@doi [\prd] {10.1103/PhysRevD.100.063519}, \href {https://ui.adsabs.harvard.edu/abs/2019PhRvD.100f3519P} {100, 063519}

\bibitem[\protect\citeauthoryear{{Perlman}, {Horner}, {Jones}, {Scharf}, {Ebeling}, {Wegner}  \& {Malkan}}{{Perlman} et~al.}{2002}]{Perlman2002}
{Perlman} E.~S.,  {Horner} D.~J.,  {Jones} L.~R.,  {Scharf} C.~A.,  {Ebeling} H.,  {Wegner} G.,   {Malkan} M.,  2002, \mn@doi [\apjs] {10.1086/339685}, \href {https://ui.adsabs.harvard.edu/abs/2002ApJS..140..265P} {140, 265}

\bibitem[\protect\citeauthoryear{{Perrott}}{{Perrott}}{2024}]{Perrott2024}
{Perrott} Y.~C.,  2024, \mn@doi [arXiv e-prints] {10.48550/arXiv.2407.16105}, \href {https://ui.adsabs.harvard.edu/abs/2024arXiv240716105P} {p. arXiv:2407.16105}

\bibitem[\protect\citeauthoryear{{Piffaretti}, {Arnaud}, {Pratt}, {Pointecouteau}  \& {Melin}}{{Piffaretti} et~al.}{2011}]{Piffaretti2011}
{Piffaretti} R.,  {Arnaud} M.,  {Pratt} G.~W.,  {Pointecouteau} E.,   {Melin} J.~B.,  2011, \mn@doi [\aap] {10.1051/0004-6361/201015377}, \href {https://ui.adsabs.harvard.edu/abs/2011A&A...534A.109P} {534, A109}

\bibitem[\protect\citeauthoryear{{Planck 2013 results XX}}{{Planck 2013 results XX}}{2014}]{Planck2014XX}
{Planck 2013 results XX} 2014, \mn@doi [\aap] {10.1051/0004-6361/201321521}, \href {https://ui.adsabs.harvard.edu/abs/2014A&A...571A..20P} {571, A20}

\bibitem[\protect\citeauthoryear{{Planck 2013 results XXIX}}{{Planck 2013 results XXIX}}{2014a}]{Planck2014}
{Planck 2013 results XXIX} 2014a, \mn@doi [\aap] {10.1051/0004-6361/201321523}, \href {http://adsabs.harvard.edu/abs/2014A%26A...571A..29P} {571, A29}

\bibitem[\protect\citeauthoryear{{Planck 2013 results XXIX}}{{Planck 2013 results XXIX}}{2014b}]{Planck2013XXIX}
{Planck 2013 results XXIX} 2014b, \mn@doi [\aap] {10.1051/0004-6361/201321523}, \href {https://ui.adsabs.harvard.edu/abs/2014A&A...571A..29P} {571, A29}

\bibitem[\protect\citeauthoryear{{Planck 2015 results VIII}}{{Planck 2015 results VIII}}{2016}]{Planck2016VIII}
{Planck 2015 results VIII} 2016, \mn@doi [\aap] {10.1051/0004-6361/201525820}, \href {https://ui.adsabs.harvard.edu/abs/2016A&A...594A...8P} {594, A8}

\bibitem[\protect\citeauthoryear{{Planck 2015 results XXIII}}{{Planck 2015 results XXIII}}{2016}]{Planck2016XXIII}
{Planck 2015 results XXIII} 2016, \mn@doi [\aap] {10.1051/0004-6361/201527418}, \href {https://ui.adsabs.harvard.edu/abs/2016A&A...594A..23P} {594, A23}

\bibitem[\protect\citeauthoryear{{Planck 2015 results XXIV}}{{Planck 2015 results XXIV}}{2016}]{Ade2016}
{Planck 2015 results XXIV} 2016, \mn@doi [\aap] {10.1051/0004-6361/201525833}, \href {http://adsabs.harvard.edu/abs/2016A%26A...594A..24P} {594, A24}

\bibitem[\protect\citeauthoryear{{Planck 2015 results XXVI}}{{Planck 2015 results XXVI}}{2016}]{Planck2015XXVI}
{Planck 2015 results XXVI} 2016, \mn@doi [\aap] {10.1051/0004-6361/201526914}, \href {https://ui.adsabs.harvard.edu/abs/2016A&A...594A..26P} {594, A26}

\bibitem[\protect\citeauthoryear{{Planck 2015 results XXVII}}{{Planck 2015 results XXVII}}{2016}]{Planck2016xxvii}
{Planck 2015 results XXVII} 2016, \mn@doi [\aap] {10.1051/0004-6361/201525823}, \href {http://adsabs.harvard.edu/abs/2016A%26A...594A..27P} {594, A27}

\bibitem[\protect\citeauthoryear{{Planck 2015 results XXVIII}}{{Planck 2015 results XXVIII}}{2016}]{Planck2015XXVIII}
{Planck 2015 results XXVIII} 2016, \mn@doi [\aap] {10.1051/0004-6361/201525819}, \href {https://ui.adsabs.harvard.edu/abs/2016A&A...594A..28P} {594, A28}

\bibitem[\protect\citeauthoryear{{Planck 2018 results III}}{{Planck 2018 results III}}{2020}]{Planck2020III}
{Planck 2018 results III} 2020, \mn@doi [\aap] {10.1051/0004-6361/201832909}, \href {https://ui.adsabs.harvard.edu/abs/2020A&A...641A...3P} {641, A3}

\bibitem[\protect\citeauthoryear{{Planck 2018 results VI}}{{Planck 2018 results VI}}{2020}]{Planck2018VI}
{Planck 2018 results VI} 2020, \mn@doi [\aap] {10.1051/0004-6361/201833910}, \href {https://ui.adsabs.harvard.edu/abs/2020A&A...641A...6P} {641, A6}

\bibitem[\protect\citeauthoryear{{Planck Collaboration}}{{Planck Collaboration}}{2014}]{Planck2014XXX}
{Planck Collaboration} 2014, \mn@doi [\aap] {10.1051/0004-6361/201322093}, \href {https://ui.adsabs.harvard.edu/abs/2014A&A...571A..30P} {571, A30}

\bibitem[\protect\citeauthoryear{{Planck intermediate results I}}{{Planck intermediate results I}}{2012}]{Planck2012I}
{Planck intermediate results I} 2012, \mn@doi [\aap] {10.1051/0004-6361/201118731}, \href {https://ui.adsabs.harvard.edu/abs/2012A&A...543A.102P} {543, A102}

\bibitem[\protect\citeauthoryear{{Planck intermediate results XI.}}{{Planck intermediate results XI.}}{2013}]{Planck2013XI}
{Planck intermediate results XI.} 2013, \mn@doi [\aap] {10.1051/0004-6361/201220941}, \href {https://ui.adsabs.harvard.edu/abs/2013A&A...557A..52P} {557, A52}

\bibitem[\protect\citeauthoryear{{Planck intermediate results XLIII.}}{{Planck intermediate results XLIII.}}{2016}]{Planck2016XLIII}
{Planck intermediate results XLIII.} 2016, \mn@doi [\aap] {10.1051/0004-6361/201628522}, \href {https://ui.adsabs.harvard.edu/abs/2016A&A...596A.104P} {596, A104}

\bibitem[\protect\citeauthoryear{{Refregier}, {Komatsu}, {Spergel}  \& {Pen}}{{Refregier} et~al.}{2000}]{Refregier2000}
{Refregier} A.,  {Komatsu} E.,  {Spergel} D.~N.,   {Pen} U.-L.,  2000, \mn@doi [\prd] {10.1103/PhysRevD.61.123001}, \href {https://ui.adsabs.harvard.edu/abs/2000PhRvD..61l3001R} {61, 123001}

\bibitem[\protect\citeauthoryear{{Remazeilles}, {Bolliet}, {Rotti}  \& {Chluba}}{{Remazeilles} et~al.}{2019}]{Remazeilles2019}
{Remazeilles} M.,  {Bolliet} B.,  {Rotti} A.,   {Chluba} J.,  2019, \mn@doi [\mnras] {10.1093/mnras/sty3352}, \href {https://ui.adsabs.harvard.edu/abs/2019MNRAS.483.3459R} {483, 3459}

\bibitem[\protect\citeauthoryear{{Repp} \& {Ebeling}}{{Repp} \& {Ebeling}}{2018}]{Repp2018}
{Repp} A.,  {Ebeling} H.,  2018, \mn@doi [\mnras] {10.1093/mnras/sty1489}, \href {https://ui.adsabs.harvard.edu/abs/2018MNRAS.479..844R} {479, 844}

\bibitem[\protect\citeauthoryear{{Romer} et~al.,}{{Romer} et~al.}{2000}]{Romer2000}
{Romer} A.~K.,  et~al., 2000, \mn@doi [\apjs] {10.1086/313302}, \href {https://ui.adsabs.harvard.edu/abs/2000ApJS..126..209R} {126, 209}

\bibitem[\protect\citeauthoryear{{Rotti} \& {Chluba}}{{Rotti} \& {Chluba}}{2021}]{Rotti2021}
{Rotti} A.,  {Chluba} J.,  2021, \mn@doi [\mnras] {10.1093/mnras/staa3292}, \href {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500..976R} {500, 976}

\bibitem[\protect\citeauthoryear{{Rotti}, {Bolliet}, {Chluba}  \& {Remazeilles}}{{Rotti} et~al.}{2021}]{Rotti2021Giants}
{Rotti} A.,  {Bolliet} B.,  {Chluba} J.,   {Remazeilles} M.,  2021, \mn@doi [\mnras] {10.1093/mnras/stab469}, \href {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503.5310R} {503, 5310}

\bibitem[\protect\citeauthoryear{{Sadibekova}, {Arnaud}, {Pratt}, {Tarr{\'\i}o}  \& {Melin}}{{Sadibekova} et~al.}{2024}]{Sadibekova2024}
{Sadibekova} T.,  {Arnaud} M.,  {Pratt} G.~W.,  {Tarr{\'\i}o} P.,   {Melin} J.~B.,  2024, \mn@doi [arXiv e-prints] {10.48550/arXiv.2402.01538}, \href {https://ui.adsabs.harvard.edu/abs/2024arXiv240201538S} {p. arXiv:2402.01538}

\bibitem[\protect\citeauthoryear{{Salvati}, {Douspis}  \& {Aghanim}}{{Salvati} et~al.}{2018}]{Salvati2018}
{Salvati} L.,  {Douspis} M.,   {Aghanim} N.,  2018, \mn@doi [\aap] {10.1051/0004-6361/201731990}, \href {https://ui.adsabs.harvard.edu/abs/2018A&A...614A..13S} {614, A13}

\bibitem[\protect\citeauthoryear{{Salvati} et~al.,}{{Salvati} et~al.}{2022}]{Salvati2022}
{Salvati} L.,  et~al., 2022, \mn@doi [\apj] {10.3847/1538-4357/ac7ab4}, \href {https://ui.adsabs.harvard.edu/abs/2022ApJ...934..129S} {934, 129}

\bibitem[\protect\citeauthoryear{{S{\'a}nchez} et~al.,}{{S{\'a}nchez} et~al.}{2023}]{Sanchez2023}
{S{\'a}nchez} J.,  et~al., 2023, \mn@doi [\mnras] {10.1093/mnras/stad1167}, \href {https://ui.adsabs.harvard.edu/abs/2023MNRAS.522.3163S} {522, 3163}

\bibitem[\protect\citeauthoryear{{Sazonov} \& {Sunyaev}}{{Sazonov} \& {Sunyaev}}{1998}]{Sazonov1998}
{Sazonov} S.~Y.,  {Sunyaev} R.~A.,  1998, \mn@doi [\apj] {10.1086/306406}, \href {http://adsabs.harvard.edu/abs/1998ApJ...508....1S} {508, 1}

\bibitem[\protect\citeauthoryear{{Spurio Mancini}, {Piras}, {Alsing}, {Joachimi}  \& {Hobson}}{{Spurio Mancini} et~al.}{2022}]{Spurio2022}
{Spurio Mancini} A.,  {Piras} D.,  {Alsing} J.,  {Joachimi} B.,   {Hobson} M.~P.,  2022, \mn@doi [\mnras] {10.1093/mnras/stac064}, \href {https://ui.adsabs.harvard.edu/abs/2022MNRAS.511.1771S} {511, 1771}

\bibitem[\protect\citeauthoryear{{Stein}, {Alvarez}  \& {Bond}}{{Stein} et~al.}{2019}]{Stein2019}
{Stein} G.,  {Alvarez} M.~A.,   {Bond} J.~R.,  2019, \mn@doi [\mnras] {10.1093/mnras/sty3226}, \href {https://ui.adsabs.harvard.edu/abs/2019MNRAS.483.2236S} {483, 2236}

\bibitem[\protect\citeauthoryear{{Stein}, {Alvarez}, {Bond}, {van Engelen}  \& {Battaglia}}{{Stein} et~al.}{2020}]{Stein2020}
{Stein} G.,  {Alvarez} M.~A.,  {Bond} J.~R.,  {van Engelen} A.,   {Battaglia} N.,  2020, \mn@doi [\jcap] {10.1088/1475-7516/2020/10/012}, \href {https://ui.adsabs.harvard.edu/abs/2020JCAP...10..012S} {2020, 012}

\bibitem[\protect\citeauthoryear{{Streblyanska}, {Barrena}, {Rubi{\~n}o-Mart{\'\i}n}, {van der Burg}, {Aghanim}, {Aguado-Barahona}, {Ferragamo}  \& {Lietzen}}{{Streblyanska} et~al.}{2018}]{Streblyanska2018}
{Streblyanska} A.,  {Barrena} R.,  {Rubi{\~n}o-Mart{\'\i}n} J.~A.,  {van der Burg} R.~F.~J.,  {Aghanim} N.,  {Aguado-Barahona} A.,  {Ferragamo} A.,   {Lietzen} H.,  2018, \mn@doi [\aap] {10.1051/0004-6361/201732306}, \href {https://ui.adsabs.harvard.edu/abs/2018A&A...617A..71S} {617, A71}

\bibitem[\protect\citeauthoryear{{Streblyanska}, {Aguado-Barahona}, {Ferragamo}, {Barrena}, {Rubi{\~n}o-Mart{\'\i}n}, {Tramonte}, {Genova-Santos}  \& {Lietzen}}{{Streblyanska} et~al.}{2019}]{Streblyanska2019}
{Streblyanska} A.,  {Aguado-Barahona} A.,  {Ferragamo} A.,  {Barrena} R.,  {Rubi{\~n}o-Mart{\'\i}n} J.~A.,  {Tramonte} D.,  {Genova-Santos} R.~T.,   {Lietzen} H.,  2019, \mn@doi [\aap] {10.1051/0004-6361/201935674}, \href {https://ui.adsabs.harvard.edu/abs/2019A&A...628A..13S} {628, A13}

\bibitem[\protect\citeauthoryear{{Sunyaev} \& {Zeldovich}}{{Sunyaev} \& {Zeldovich}}{1972}]{Sunyaev1972}
{Sunyaev} R.~A.,  {Zeldovich} Y.~B.,  1972, Comments on Astrophysics and Space Physics, \href {http://adsabs.harvard.edu/abs/1972CoASP...4..173S} {4, 173}

\bibitem[\protect\citeauthoryear{{Tarr{\'\i}o}, {Melin}  \& {Arnaud}}{{Tarr{\'\i}o} et~al.}{2019}]{Tarrio2019}
{Tarr{\'\i}o} P.,  {Melin} J.~B.,   {Arnaud} M.,  2019, \mn@doi [\aap] {10.1051/0004-6361/201834979}, \href {https://ui.adsabs.harvard.edu/abs/2019A&A...626A...7T} {626, A7}

\bibitem[\protect\citeauthoryear{{Tinker}, {Kravtsov}, {Klypin}, {Abazajian}, {Warren}, {Yepes}, {Gottl{\"o}ber}  \& {Holz}}{{Tinker} et~al.}{2008}]{Tinker2008}
{Tinker} J.,  {Kravtsov} A.~V.,  {Klypin} A.,  {Abazajian} K.,  {Warren} M.,  {Yepes} G.,  {Gottl{\"o}ber} S.,   {Holz} D.~E.,  2008, \mn@doi [\apj] {10.1086/591439}, \href {http://adsabs.harvard.edu/abs/2008ApJ...688..709T} {688, 709}

\bibitem[\protect\citeauthoryear{{Vacher}, {Chluba}, {Aumont}, {Rotti}  \& {Montier}}{{Vacher} et~al.}{2022}]{Vacher2022a}
{Vacher} L.,  {Chluba} J.,  {Aumont} J.,  {Rotti} A.,   {Montier} L.,  2022, arXiv e-prints, \href {https://ui.adsabs.harvard.edu/abs/2022arXiv220501049V} {p. arXiv:2205.01049}

\bibitem[\protect\citeauthoryear{{Vanderlinde}, {Crawford}, {de Haan}, {Dudley}, {Shaw}  et~al.}{{Vanderlinde} et~al.}{2010}]{Vanderlinde2010}
{Vanderlinde} K.,  {Crawford} T.~M.,  {de Haan} T.,  {Dudley} J.~P.,  {Shaw} L.,   et~al., 2010, \mn@doi [\apj] {10.1088/0004-637X/722/2/1180}, \href {https://ui.adsabs.harvard.edu/abs/2010ApJ...722.1180V} {722, 1180}

\bibitem[\protect\citeauthoryear{{Weinberg}, {Mortonson}, {Eisenstein}, {Hirata}, {Riess}  \& {Rozo}}{{Weinberg} et~al.}{2013}]{Weinberg13}
{Weinberg} D.~H.,  {Mortonson} M.~J.,  {Eisenstein} D.~J.,  {Hirata} C.,  {Riess} A.~G.,   {Rozo} E.,  2013, \mn@doi [\physrep] {10.1016/j.physrep.2013.05.001}, \href {https://ui.adsabs.harvard.edu/abs/2013PhR...530...87W} {530, 87}

\bibitem[\protect\citeauthoryear{{Xu}, {Ramos-Ceja}, {Pacaud}, {Reiprich}  \& {Erben}}{{Xu} et~al.}{2022}]{Xu2022}
{Xu} W.,  {Ramos-Ceja} M.~E.,  {Pacaud} F.,  {Reiprich} T.~H.,   {Erben} T.,  2022, \mn@doi [\aap] {10.1051/0004-6361/202140908}, \href {https://ui.adsabs.harvard.edu/abs/2022A&A...658A..59X} {658, A59}

\bibitem[\protect\citeauthoryear{{Yan}, {Hojjati}, {Tr{\"o}ster}, {Hinshaw}  \& {van Waerbeke}}{{Yan} et~al.}{2019}]{Yan2019}
{Yan} Z.,  {Hojjati} A.,  {Tr{\"o}ster} T.,  {Hinshaw} G.,   {van Waerbeke} L.,  2019, \mn@doi [\apj] {10.3847/1538-4357/ab40b2}, \href {https://ui.adsabs.harvard.edu/abs/2019ApJ...884..139Y} {884, 139}

\bibitem[\protect\citeauthoryear{{Zaznobin} et~al.,}{{Zaznobin} et~al.}{2019}]{Zaznobin2019}
{Zaznobin} I.~A.,  et~al., 2019, \mn@doi [Astronomy Letters] {10.1134/S1063773719020063}, \href {https://ui.adsabs.harvard.edu/abs/2019AstL...45...49Z} {45, 49}

\bibitem[\protect\citeauthoryear{{Zaznobin} et~al.,}{{Zaznobin} et~al.}{2020}]{Zaznobin2020}
{Zaznobin} I.~A.,  et~al., 2020, \mn@doi [Astronomy Letters] {10.1134/S1063773720020048}, \href {https://ui.adsabs.harvard.edu/abs/2020AstL...46...79Z} {46, 79}

\bibitem[\protect\citeauthoryear{{Zohren}, {Schrabback}, {van der Burg}, {Arnaud}, {Melin}, {van den Busch}, {Hoekstra}  \& {Klein}}{{Zohren} et~al.}{2019}]{Zohren2019}
{Zohren} H.,  {Schrabback} T.,  {van der Burg} R. F.~J.,  {Arnaud} M.,  {Melin} J.-B.,  {van den Busch} J.~L.,  {Hoekstra} H.,   {Klein} M.,  2019, \mn@doi [\mnras] {10.1093/mnras/stz1838}, \href {https://ui.adsabs.harvard.edu/abs/2019MNRAS.488.2523Z} {488, 2523}

\bibitem[\protect\citeauthoryear{{Zubeldia}}{{Zubeldia}}{2024}]{Zubeldia2024Grenoble}
{Zubeldia} {\'I}.,  2024, in European Physical Journal Web of Conferences. p. 00053, \mn@doi{10.1051/epjconf/202429300053}

\bibitem[\protect\citeauthoryear{{Zubeldia} \& {Bolliet}}{{Zubeldia} \& {Bolliet}}{2024}]{Zubeldia2024}
{Zubeldia} {\'I}.,  {Bolliet} B.,  2024, \mn@doi [arXiv e-prints] {10.48550/arXiv.2403.09589}, \href {https://ui.adsabs.harvard.edu/abs/2024arXiv240309589Z} {p. arXiv:2403.09589}

\bibitem[\protect\citeauthoryear{{Zubeldia} \& {Challinor}}{{Zubeldia} \& {Challinor}}{2019}]{Zubeldia2019}
{Zubeldia} {\'{I}}.,  {Challinor} A.,  2019, \mn@doi [\mnras] {10.1093/mnras/stz2153}, \href {https://ui.adsabs.harvard.edu/abs/2019MNRAS.489..401Z} {489, 401}

\bibitem[\protect\citeauthoryear{{Zubeldia}, {Rotti}, {Chluba}  \& {Battye}}{{Zubeldia} et~al.}{2021}]{Zubeldia2021}
{Zubeldia} {\'I}.,  {Rotti} A.,  {Chluba} J.,   {Battye} R.,  2021, \mn@doi [\mnras] {10.1093/mnras/stab2461}, \href {https://ui.adsabs.harvard.edu/abs/2021MNRAS.507.4852Z} {507, 4852}

\bibitem[\protect\citeauthoryear{{Zubeldia}, {Rotti}, {Chluba}  \& {Battye}}{{Zubeldia} et~al.}{2023a}]{Zubeldia2022}
{Zubeldia} {\'I}.,  {Rotti} A.,  {Chluba} J.,   {Battye} R.,  2023a, \mn@doi [\mnras] {10.1093/mnras/stad1320}, \href {https://ui.adsabs.harvard.edu/abs/2023MNRAS.522.4766Z} {522, 4766}

\bibitem[\protect\citeauthoryear{{Zubeldia}, {Chluba}  \& {Battye}}{{Zubeldia} et~al.}{2023b}]{Zubeldia2023}
{Zubeldia} {\'I}.,  {Chluba} J.,   {Battye} R.,  2023b, \mn@doi [\mnras] {10.1093/mnras/stad1318}, \href {https://ui.adsabs.harvard.edu/abs/2023MNRAS.522.5123Z} {522, 5123}

\bibitem[\protect\citeauthoryear{{van der Burg} et~al.,}{{van der Burg} et~al.}{2016}]{vanderBurg2016}
{van der Burg} R.~F.~J.,  et~al., 2016, \mn@doi [\aap] {10.1051/0004-6361/201527299}, \href {https://ui.adsabs.harvard.edu/abs/2016A&A...587A..23V} {587, A23}

\bibitem[\protect\citeauthoryear{{van der Burg}, {McGee}, {Aussel}, {Dahle}, {Arnaud}, {Pratt}  \& {Muzzin}}{{van der Burg} et~al.}{2018}]{vanderBurg2018}
{van der Burg} R. F.~J.,  {McGee} S.,  {Aussel} H.,  {Dahle} H.,  {Arnaud} M.,  {Pratt} G.~W.,   {Muzzin} A.,  2018, \mn@doi [\aap] {10.1051/0004-6361/201833572}, \href {https://ui.adsabs.harvard.edu/abs/2018A&A...618A.140V} {618, A140}

\makeatother
\end{thebibliography}

